Federated Agentic AI for Interference-Aware Adaptive Spectrum Coordination

Emerging intelligent wireless networks increasingly rely on autonomous AI agents to adapt spectrum usage to dynamic and heterogeneous operating conditions. However, collective learning is challenging when agents experience different local interference environments and cannot exchange raw observations due to communication-overhead and privacy constraints. We propose Federated Agentic Spectrum Coordination with Interference Awareness (FASCIA), a federated multi-agent deep reinforcement learning framework for adaptive spectrum coordination. In FASCIA, each network manager acts as an autonomous AI agent that perceives its local interference environment, accumulates experience in a persistent local memory, and learns an adaptive spectrum coordination policy through local interactions. Coordination among agents is achieved through periodic federated aggregation of locally trained models, without exchanging raw sensing data or experience. Since spectrum decisions made by one agent alter the environments observed by others, local learning is inherently heterogeneous and coupled. FASCIA employs proximal regularization to mitigate the resulting model drift and explicitly accounts for inter-carrier interference arising from partially overlapping channels. FASCIA is the first federated agentic AI framework to address this challenging interference-coupled spectrum coordination setting. Extensive simulations demonstrate that FASCIA achieves performance close to the centralized benchmark while avoiding raw-experience exchange and maintaining effectiveness across heterogeneous network configurations.

==> figs/tikz/fig_e_sweep.tex <==
% Editable PGFPlots: FedProx E-sweep (discrete markers, no connecting lines).
% Data: figs/data/e_sweep.csv
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=1.35cm},
  width=0.50\columnwidth, height=0.42\columnwidth,
  grid=major, grid style={gray!25},
  xlabel={Local steps $E$},
  xlabel style={yshift=-2pt},
  xtick={0,...,11},
  xticklabels={1,{},5,10,{},20,{},60,{},120,{},300},
  x tick label style={font=\tiny, rotate=0, anchor=north},
  tick label style={font=\scriptsize},
  label style={font=\small},
  table/col sep=comma,
  enlarge x limits=0.06,
]
\nextgroupplot[
  ylabel={$\mathbb{E}[(\mathrm{CQ}+\min_{\mathrm{CQ}})/2]$},
  ymin=0.978, ymax=0.997,
]
  \addplot+[
    only marks, mark=*, mark size=2.0pt, cbFedProx,
    error bars/.cd, y dir=both, y explicit, error bar style={line width=0.6pt}
  ]
    table[x expr=\coordindex, y=composite_mean, y error=composite_std]
    {figs/data/e_sweep.csv};
  \draw[gray, dashed, thin] (axis cs:3,0.978) -- (axis cs:3,0.997);
  \node[font=\tiny, gray!50!black, anchor=north] at (axis cs:3,0.9965) {$E{=}10$};

\nextgroupplot[
  ylabel={Throughput [Mbps]},
  ymin=12.2, ymax=15.6,
]
  \addplot+[
    only marks, mark=square*, mark size=2.0pt, cbFedAvg,
    error bars/.cd, y dir=both, y explicit, error bar style={line width=0.6pt}
  ]
    table[x expr=\coordindex, y=rate_mean, y error=rate_std]
    {figs/data/e_sweep.csv};
  \draw[gray, dashed, thin] (axis cs:3,12.2) -- (axis cs:3,15.6);
\end{groupplot}
\end{tikzpicture}


==> figs/tikz/fig_fig13_vs_n.tex <==
% Editable PGFPlots: composite CQ vs number of networks.
% Labels: figs/tikz/plot_labels.tex   Data: figs/data/fig13_vs_n.csv
\begin{tikzpicture}
\begin{axis}[
  width=0.95\columnwidth,
  height=0.58\columnwidth,
  xlabel={Number of networks $N$},
  ylabel={$\mathbb{E}[(\mathrm{CQ}+\min\mathrm{CQ})/2]$},
  label style={font=\small},
  tick label style={font=\scriptsize},
  xmin=1.5, xmax=15.5,
  ymin=0.15, ymax=1.08,
  xtick={2,4,6,7,8,10,12,14},
  grid=major, grid style={gray!25},
  % Legend ABOVE the axes so it never overlaps the curves.
  legend style={
    at={(0.5,1.02)}, anchor=south,
    legend columns=-1,
    font=\scriptsize, draw=none, fill=none,
    /tikz/every even column/.append style={column sep=0.18cm}
  },
  legend cell align=left,
  every mark/.append style={solid},
  error bars/error bar style={opacity=0.45, line width=0.5pt},
]
% Distinct color + marker + line style (readable without color).
\addplot+[thick, solid, mark=*, mark size=1.5pt, cbCTDE,
  error bars/.cd, y dir=both, y explicit]
  table[x=N, y=CTDE, y error=CTDE_std, col sep=comma] {figs/data/fig13_vs_n.csv};
\addlegendentry{\PlotLabelCTDE}
\addplot+[thick, dashed, mark=square*, mark size=1.4pt, cbFedAvg,
  error bars/.cd, y dir=both, y explicit]
  table[x=N, y=FedAvg, y error=FedAvg_std, col sep=comma] {figs/data/fig13_vs_n.csv};
\addlegendentry{\PlotLabelFedAvg}
\addplot+[thick, dashdotted, mark=triangle*, mark size=1.6pt, cbFedProx,
  error bars/.cd, y dir=both, y explicit]
  table[x=N, y=FedProx, y error=FedProx_std, col sep=comma] {figs/data/fig13_vs_n.csv};
\addlegendentry{\PlotLabelFedProx}
\addplot+[thick, densely dotted, mark=diamond*, mark size=1.5pt, cbJAR,
  error bars/.cd, y dir=both, y explicit]
  table[x=N, y=JAR, y error=JAR_std, col sep=comma] {figs/data/fig13_vs_n.csv};
\addlegendentry{\PlotLabelJAR}
\addplot+[thick, loosely dashed, mark=o, mark size=1.5pt, cbRA,
  error bars/.cd, y dir=both, y explicit]
  table[x=N, y=RA, y error=RA_std, col sep=comma] {figs/data/fig13_vs_n.csv};
\addlegendentry{\PlotLabelRA}
\draw[dashed, gray, thin] (axis cs:7.5,0.15) -- (axis cs:7.5,1.08);
\node[font=\scriptsize, gray!55!black, anchor=north east]
  at (axis cs:7.35,0.22) {in-sample};
\node[font=\scriptsize, gray!55!black, anchor=north west]
  at (axis cs:7.65,0.22) {out-of-sample};
\end{axis}
\end{tikzpicture}


==> figs/tikz/fig_fig15_bars.tex <==
% Editable PGFPlots: Fig.15-style in/out composite bars.
% Labels: figs/tikz/plot_labels.tex   Data: figs/data/fig15_bars_wide.csv
\begin{tikzpicture}
\begin{axis}[
  width=0.95\columnwidth,
  height=0.60\columnwidth,
  ybar=1.5pt,
  bar width=5.5pt,
  enlarge x limits=0.28,
  symbolic x coords={In,Out},
  xtick=data,
  xticklabels={
    {In-sample\\($N\leq 7$)},
    {Out-of-sample\\($N>7$)}
  },
  xticklabel style={align=center, font=\scriptsize},
  ylabel={$\mathbb{E}[(\mathrm{CQ}+\min\mathrm{CQ})/2]$},
  ylabel style={font=\small},
  ymin=0, ymax=1.28,
  grid=major, grid style={gray!25},
  legend style={
    at={(0.5,1.01)}, anchor=south, legend columns=-1,
    font=\scriptsize, draw=none,
    /tikz/every even column/.append style={column sep=0.18cm}
  },
  nodes near coords={\pgfmathprintnumber[fixed,precision=2]{\pgfplotspointmeta}},
  every node near coord/.append style={
    font=\tiny,
    rotate=90,
    anchor=west,
    inner sep=1pt
  },
]
\addplot[fill=cbCTDE, draw=none]
  table[x=setting, y=CTDE, col sep=comma] {figs/data/fig15_bars_wide.csv};
\addplot[fill=cbFedAvg, draw=none]
  table[x=setting, y=FedAvg, col sep=comma] {figs/data/fig15_bars_wide.csv};
\addplot[fill=cbFedProx, draw=none]
  table[x=setting, y=FedProx, col sep=comma] {figs/data/fig15_bars_wide.csv};
\addplot[fill=cbJAR, draw=none]
  table[x=setting, y=JAR, col sep=comma] {figs/data/fig15_bars_wide.csv};
\addplot[fill=cbRA, draw=none]
  table[x=setting, y=RA, col sep=comma] {figs/data/fig15_bars_wide.csv};
\legend{\PlotLabelCTDE,\PlotLabelFedAvg,\PlotLabelFedProx,\PlotLabelJAR,\PlotLabelRA}
\end{axis}
\end{tikzpicture}


==> figs/tikz/fig_throughput.tex <==
% Editable PGFPlots: Shannon throughput vs round (dual panel).
% Labels: figs/tikz/plot_labels.tex
% Data: figs/data/throughput_fedavg.csv, throughput_fedprox.csv
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=1.45cm},
  width=0.49\columnwidth, height=0.40\columnwidth,
  grid=major, grid style={gray!25},
  xlabel={Training round},
  tick label style={font=\scriptsize},
  label style={font=\small},
  legend style={font=\scriptsize, draw=none, at={(0.03,0.97)}, anchor=north west},
  table/col sep=comma,
  xtick={0,250,500,750,1000},
  error bars/error bar style={opacity=0.5, line width=0.5pt},
  every mark/.append style={solid},
]
\nextgroupplot[ylabel={Throughput [Mbps]}, title={(a)}, ymin=7.5, ymax=11.2]
  \addplot+[thick, solid, mark=*, mark size=1.2pt, cbFedAvg,
    error bars/.cd, y dir=both, y explicit]
    table[x=round, y=mean_smooth, y error=std] {figs/data/throughput_fedavg.csv};
  \addlegendentry{\PlotLabelFedAvg}
  \addplot+[thick, dashed, mark=square*, mark size=1.2pt, cbFedProx,
    error bars/.cd, y dir=both, y explicit]
    table[x=round, y=mean_smooth, y error=std] {figs/data/throughput_fedprox.csv};
  \addlegendentry{\PlotLabelFedProx}

\nextgroupplot[ylabel={$R(t)/R(T)$}, title={(b)}, ymin=0.55, ymax=1.08]
  \addplot+[thick, solid, mark=*, mark size=1.2pt, cbFedAvg]
    table[x=round, y=norm_smooth] {figs/data/throughput_fedavg.csv};
  \addplot+[thick, dashed, mark=square*, mark size=1.2pt, cbFedProx]
    table[x=round, y=norm_smooth] {figs/data/throughput_fedprox.csv};
\end{groupplot}
\end{tikzpicture}


==> figs/tikz/plot_labels.tex <==
%==============================================================================
% Editable plot labels + colorblind-safe series styles (Okabe–Ito).
% Edit the names below; all campaign TikZ figures pick them up automatically.
%==============================================================================
\newcommand{\PlotLabelCTDE}{CTDE}
\newcommand{\PlotLabelFedAvg}{\FedAvg{}}
\newcommand{\PlotLabelFedProx}{\FedProx{}}
\newcommand{\PlotLabelJAR}{JAR}
\newcommand{\PlotLabelRA}{RA}

% Okabe–Ito palette (colorblind-friendly)
\definecolor{cbCTDE}{HTML}{0072B2}
\definecolor{cbFedAvg}{HTML}{E69F00}
\definecolor{cbFedProx}{HTML}{009E73}
\definecolor{cbJAR}{HTML}{D55E00}
\definecolor{cbRA}{HTML}{CC79A7}
\definecolor{cbAccentA}{HTML}{56B4E9}
\definecolor{cbAccentB}{HTML}{F0E442}

